Nuclear Forces for Precision Nuclear Physics -- a collection of perspectives

This is a collection of perspective pieces contributed by the participants of the Institute of Nuclear Theory's Program on Nuclear Physics for Precision Nuclear Physics which was held virtually from April 19 to May 7, 2021. The collection represents the reflections of a vibrant and engaged community of researchers on the status of theoretical research in low-energy nuclear physics, the challenges ahead, and new ideas and strategies to make progress in nuclear structure and reaction physics, effective field theory, lattice QCD, quantum information, and quantum computing. The contributed pieces solely reflect the perspectives of the respective authors and do not represent the viewpoints of the Institute for Nuclear theory or the organizers of the program.

==> bibliography.tex <==
%% the following lines add a Bibliography to the end of the document. This is in addition to the chapter-specific References sections
\cleardoublepage
\addtocontents{toc}{\protect\setcounter{tocdepth}{1}}
\nocite{*}
\appto{\bibfont}{\footnotesize}
\begin{multicols}{2}
\printbibliography[env=nolabelbib,title={Bibliography},heading=bibintoc]
\end{multicols}

